Goal Recognition using Actor-Critic Optimization

Goal Recognition aims to infer an agent's goal from a sequence of observations. Existing approaches often rely on manually engineered domains and discrete representations. Deep Recognition using Actor-Critic Optimization (DRACO) is a novel approach based on deep reinforcement learning that overcomes these limitations by providing two key contributions. First, it is the first goal recognition algorithm that learns a set of policy networks from unstructured data and uses them for inference. Second, DRACO introduces new metrics for assessing goal hypotheses through continuous policy representations. DRACO achieves state-of-the-art performance for goal recognition in discrete settings while not using the structured inputs used by existing approaches. Moreover, it outperforms these approaches in more challenging, continuous settings at substantially reduced costs in both computing and memory. Together, these results showcase the robustness of the new algorithm, bridging traditional goal recognition and deep reinforcement learning.

==> sections/definitions.tex <==
% !TEX root = ../main.tex
% \begin{definition}
% \label{def:MDP}
% \textbf{(MDP)} A \textbf{Markov Decision Process} M, is a
% 4-tuple $(S, A, p, r)$ such that $S$ are the possible states in the
% environment, $A$ is the set of actions the actor can execute, $P(s' \mid s, a)$ is a transition function that gives the probability of transitioning from state s to state $s'$ after taking action $a$
% and $r(s, a, s')$ defines a reward function.

% One of the capabilities of MDPs is that they can represent the behavior of an agent in a stochastic environment that follows the assumption that outcomes are partly random and partly under the control of the decision-maker. 
% \end{definition}

% \begin{definition}
% \label{def:Policy}
% \textbf{Policy $\pi(a \mid s) $ } A policy for an MDP is a function that defines the probability of the agent taking action $a \in A$ in state $s \in S$. Some RL algorithms, such as Q-learning, compute the policy of an agent using a Q-function Q(s, a), which is an
% estimation of the expected rewards of all future steps starting from s after taking action a. However, AC computes the policy using the actor-network, which returns the probability of taking each action in the specific state (the policy).
% \end{definition}


We use a similar formulation for a goal recognition problem as Ramirez and Geffner \shortcite{ramirez2009plan}:

\begin{definition}
    A \textit{Goal Recognition (GR)} problem. Given a set of possible goals $G$, and observations $O$, an IR problem outputs a goal $g \in G$ that $O$ explains.
\end{definition}

As we consider an extended version of GR with AR, both the goal and the observations can be viewed as a symbolic state representation (e.g., coordinates in space) as well as images or other raw data. Each goal $g$ can be expressed as a set of labels over possible goal states, or a probability distribution over alternative sets of these states. Similarly, the observations $O$ can be either a sequence of symbolic states or raw data. In addition, the observations can be fully or partly specified, meaning whether all actions and state sets are given to the observer or only part of them.



==> sections/diff-DRACO.tex <==
% !TEX root = ../main.tex
% The approach taken in this work uses an off-the-self data-driven DRL algorithm family called Actor-Critic (AC) \cite{schulman2017proximal} to perform GR.

\begin{figure*}[t]
    \centering
        \includegraphics[width=0.9\textwidth]{Figures/DRACO_3_obs.pdf}
       \caption{A description of DRACO's processes. 
       %The algorithm receives a set of goals, out of which it learns a set of policies for reaching each goal (Section \ref{sec:learn}). Then, given an observation sequence, the algorithm computes the likelihood of each goal to explain the observation sequence (Section \ref{sec:infer}) to output a probability distribution describing how likely is each goal to be the goal the agent is pursuing.
       %%% FRM - I removed the long description because this was repetition of what we already had in 3.
       } 
       \label{fig:draco}
       \reuth[inline]{Changed the figure to have three observations. Should we also add in writing that the top grid on the right is $g_1$ and the bottom one is $g_2$, or is it clear?}
\end{figure*}

This section introduces our new algorithm for goal recognition: Deep Recognition using Actor-Critic Optimization (DRACO).
DRACO relies on the assumption from reinforcement learning that the environment behaves as an MDP, yet in practice, we only need to represent states and actions as our domain theory $\planningdomain$ from Definition \ref{def:GR}. 
Formally, in this work, a \DIFdelbegin \DIFdel{goal recognition }\DIFdelend \DIFaddbegin \DIFadd{GR }\DIFaddend problem is a triple $\tuple{\planningdomain,G,O}$ where:
\begin{itemize}
    \item $\planningdomain=\tuple{\states, \actions}$ is a set of states and actions, both of which can be discrete or continuous, \DIFdelbegin \DIFdel{meaning that }\DIFdelend $\states \subseteq \Real^{n}$ and $\actions \subseteq \Real^{n}$; 
    \item $\goals \subseteq \states$ is a set of potential goals, out of which we assume the \DIFdelbegin \DIFdel{actor }\DIFdelend \DIFaddbegin \DIFadd{effectuator }\DIFaddend pursues exactly one; and
    \item $\observations = s_0, a_0, s_1, a_1, s_2, a_2, \ldots$ is a sequence of state-action observations, such that $s_i \in S$ and $a_i \in A$.
\end{itemize}


This definition is purposefully broad to allow for different possible instantiations of the problem. 
Thus, states can be images or continuous data such as a robot's joints' location and velocities. This state representation obviates the need for manually prescribing labels or symbols to specific states. %with actions being similarly broad. 
Additionally, while we do not assume explicit transition dynamics to be part of the problem, we assume we have access to the environment or to some model $\model$ of the environment, such as a sampling model or simulator. 
This assumption frees us from explicitly prescribing action dynamics as part of a recognition problem and steers our focus to solutions that are based on model-free RL techniques. 

% As a goal recognition algorithm, DRACO is required to reason about which goal is most likely to explain a set of observations. It does so by comparing this sequence to policies, such that each policy represents one possible goal from $G$. 

Figure~\ref{fig:draco} illustrates the recognition process using DRACO, which we explain in this section. 
DRACO starts by receiving a set of goals, where in the figure $|\goals|=2$ and the observation sequence $O$ consists of three observations. 
To solve the GR problem, Section \ref{sec:learn} discusses how DRACO first learns a set of policies, one policy for each goal, using simulated interactions. 
Then, Section \ref{sec:infer} explains how DRACO compares the observation sequence $O$ against each of the goal-oriented policies to estimate the likelihood of the \DIFdelbegin \DIFdel{actor }\DIFdelend \DIFaddbegin \DIFadd{effectuator }\DIFaddend producing $O$ given each policy. 
Key to this comparison is the metric we use when processing observations and comparing them to policies. In this work, we propose two different metrics. 
% While previous work makes strong assumptions of discreteness, we extend these metrics to continuous domains in Section~\ref{sec:metrics}. 
The algorithm then outputs a distribution over the set of goals to represent how likely it is that each goal explains the observations.
% and is inefficient to compute more than once if the set of goals is known in advance.
% Using DRL will help us to understand the environmental details better, have fast convergence and redundant human experts and, as a result, distinguish the correct goal efficiently.



% (GRDRL\frm{I liked DRAQL. It sounds like dragon or something. And that's \textbf{manly}! Like Deep Recognition as Q-learning or something like that.}).
% Unlike the tabular learning approach from \citeauthor{amado2022goal}~\shortcite{amado2022goal}, which uses discrete structured observations and goals, we leverage actor-critic reinforcement learning to lift this limitation. \frm{We still need to say something stronger than this at this point. Did we have to adapt any of the distance metrics? I recall we had a discussion on this.} \reuth{We can add a section about the "infer" stage, but I wouldn't compare too much to GRAQL so we don't get a bad review for doing "incremental work".}
% \citeauthor{amado2022goal}~\shortcite{amado2022goal} uses the off-the-shelf Q-Learning value-based algorithm in their framework learning part. 
% Nevertheless, in this approach, the learning algorithm is replaced with AC which mixes value and policy-based algorithms.
% Replacing the tabular RL approach taken by \citeauthor{amado2022goal}~\shortcite{amado2022goal} with DRL has many advantages.

% In tabular RL, for each state and action, Q-value is memorized making it infeasible to model large and physical domains using those conventional methods. 
%factories, parks, universities, or neighborhoods.
% AC, and deep learning in general, are commonly used to solve complicated problems without defining specific features via function approximations.
% In this proposal, we exploit this function approximation to compute optimal paths to reach each goal.


% Thus, our technique exploits this function approximation to compute optimal paths to reach each goal. 
% Nevertheless, it learns from taking actions, transforming the states and actions into experiences (set of state, action, reward), and eventually having the optimal policy when encountering similar environmental settings.
% Using DRL will help us to understand the environmental details better, have fast convergence and redundant human experts and, as a result, distinguish the correct goal efficiently.



==> sections/mini-grid-diff.tex <==
% !TEX root = ../main.tex
% \reuth{elaborate on the difference in inputs for each framework, it's not just an observation sequence, that's already the second stage.}

% As mentioned before both frameworks have the same guidelines: the learning, and inferring phases.
% The two frameworks' input is the environment and an agent's observation trace (partial or full). Their observation trace consists of a sequence of 2 elements each, the environment's current state and the agent's action in this state.
% However, their current state representation differs.
% While GRDRL's input is the environment's current setting in its image representation, GRAQL's input is the agent's parsed position as vectors.


% \begin{itemize}
%     \item The number of episodes is 50k.
%     \item The discount factor ($\gamma$) is 0.99.
%     \item The learning rate ($\alpha$) is 0.001.
%     \item The $\epsilon$ used for computing $\pi_O$ is $1e^{-6}$.
% \end{itemize}




% The values of these metrics are averaged across $10$ runs per configuration.

\input{sections/minigrid-table2}
% \input{sections/minigrid-tables2}
\input{sections/minigrid-figures}
\input{sections/panda-table}
\input{sections/panda-noisy-table}

\section{Results}
% The comparison between DRACO and the GRAQL baseline has two levels: Scalability and Performance.
% To compare DRACO and the GRAQL baseline we have to equate them in two levels: Scalability and Performance.
We compare approaches in scalability and performance. 
% \ben{Added the Scalability Paragraph - feel free to modify}
{\noindent\textbf{Scalability}} has three main factors: storage, training and execution time. 
First, in terms of storage consumption, DRACO uses a constant $8 \pm 0.0$ MB while GRAQL $3190 \pm 700$ MB. 
This difference is primarily due to the huge storage needs of the Q-table used by GRAQL.
The Q-table's size depends on the hyperparameter discretization factor selection because the number of valid states and possible actions in these states increase as we decrease this factor.
% This difference derives from the usage of Q-Learning by GRAQL. Q-Learning saves a cell in its table for every unique state and action tuple, making it tremendously heavy especially for large domains like Panda-Gym. 
By contrast,  DRACO uses constant memory because it stores only the network architecture and neurons' values. Even though, these neurons' values change along the training time their memory consumption remains constant.
% However, DRACO uses constant memory because it stores only the network architecture and neurons' values. 
% In terms of the second factor of scalability, execution time, 
Second, DRACO's average training time was $13.52 \pm  4.3$ minutes while GRAQL's was $1108 \pm 463$ minutes.
% This difference can be related to the exhaustive use of storage by GRAQL and also related to GRAQL's implementation which relies on the CPU computation only.
This difference is due to two factors: (i) GRAQL relies on the CPU for its computation, whereas DRACO uses a GPU; and (ii) GRAQL's storage-intensive operations are more expensive. 
Third, as discussed in section \ref{sec:infer}\DIFaddbegin \DIFadd{, }\DIFaddend GRAQL and DRACO compute their policies in the inference stage. During this computation, GRAQL loads the goal-dependent Q-tables. Since these Q-tables are huge, their loading time is often not negligible and takes $\approx$ 3.4 minutes per table on average while DRACO's NNs loading time takes seconds.
We trained both approaches on the same commodity Tesla K40 server.
% Note that both approaches were trained on the same commodity Tesla K40 server.


\noindent\textbf{Performance} Our tests generated observation sequences by using a different algorithm from our learning methods, namely Asynchronous Actor-Critic (A2C) \cite{mnih2016asynchronous}.
For each combination of algorithm and instance, the observation sequence $O$ %provided to the algorithms 
varies its degree of observability: $10\%$, $30\%$, $50\%$, $70\%$, and full observability. 
We generate an observation sequence with $x\%$ observability by taking a full sequence and removing each observation along the trajectory with $x\%$ probability. 
Similarly, we generate noisy observations by appending suboptimal actions to $x\%$ of the states.\footnote{Examples of non-noisy and noisy observations in supplement.} 
For each execution in every environment, we use the same trajectories for all algorithms.
Table~\ref{tab:minigrid} and Figure~\ref{fig:panda-comp} show the metrics averaged over $10$ executions with varying degrees of observability ($13$ per execution).
In total, throughout the evaluation phase, $540$ GR problem instances executed on Minigrid and Panda-Gym and their summarized results appear in Table~\ref{tab:minigrid} and Figure~\ref{fig:panda-comp}.
% , both in MiniGrid and Panda-gym. 
% For each execution we used the same trajectories in the two frameworks, removing steps randomly to achieve a specific observability ratio. 

Table~\ref{tab:minigrid} shows results for MiniGrid. 
Both approaches perform overwhelmingly well, with perfect scores on all measures when the observability is $0.5$ or higher, and under noisy observations. % or equal to 0.5, both frameworks achieved perfect scores.
However, this result is misleading: %, as both of the algorithms calculated the difference between the observation and the policy for each goal GRACO's distance measurement was more accurate.
while GRAQL's true goal score was close to the other goals' score ($5\%$ difference on average), DRACO has very different scores between the true goal and the other candidates ($20\%$ on average), making its confidence in the true goal higher. 
Moreover, DRACO's results dominate those of GRAQL in the more challenging, low observability ($10\%$, $30\%$), problem variants. 
It is a reasonable outcome because DL can make significant inroads to recognizing patterns and variance instead of valuing the current state. 
Moreover, our use of a smoothed policy for the observation sequence $O$, makes DRACO more forgiving to missing observations, as the likelihood of these missing actions \DIFdelbegin \DIFdel{in }\DIFdelend \DIFaddbegin \DIFadd{is }\DIFaddend $\epsilon$ rather than zero, and this difference accumulated with the number of missing observations.
% Lastly, when evaluating the algorithm's performance on noisy observation sequences, the results show that both GRAQL and DRACO were able to correctly identify the true goal of the agent. 
%
% However, even 
%
% However, This result is misleading, as DRACO ranked the true goal with a much higher probability than the other goals, while in GRAQL the difference between the true goal and the others was smaller.
%
Lastly, previous work has shown that GRAQL outperforms planning-based approaches that use PDDL representation. 
So while a direct comparison between DRACO and PDDL-based approaches is not trivial, a comparison to an intermediate solution (GRAQL) shows that DRACO outperforms it. 
%by matching up to the performance of GRAQL, DRACO can be considered to transitively outperform these methods as well.

% \ben{Modified it to be Figure instead of Table ~\ref{tab:panda}}  
\DIFaddbegin \DIFadd{To assess the performance of DRACO in continuous settings we first compare it to GRAQL and then discuss the different metrics proposed in section \ref{sec:infer}. 
}\DIFaddend Figure~\ref{fig:panda-comp} reports the average F-Score for all Panda-Gym problems running GRAQL in \DIFdelbegin \DIFdel{the discretized environment }\DIFdelend \DIFaddbegin \DIFadd{a discretized environment version }\DIFaddend and DRACO in the regular environment using the \DIFdelbegin \DIFdel{different  evaluation metrics proposed in section \ref{sec:infer}.
}\DIFdelend \DIFaddbegin \DIFadd{proposed evaluation metrics for inference.
Firstly, }\DIFaddend DRACO's performance is similar and often superior to GRAQL, often reaching the best results regardless of the distance metric used\DIFdelbegin \DIFdel{under the environment 
}\DIFdelend \DIFaddbegin \DIFadd{. These Figures illustrate GRAQL's difficulty in generalizing continuous and relatively large environments. It happens due to one of the main differences between DL and tabular methods - DL learns from similar states while Q-Learning doesn't, affecting the number of episodes GRAQL requires to learn a problem.
}\DIFaddend Recall that DRACO with PPO was consistently better than DRACO with SAC. 
However, PPO converges to a less optimal policy for each goal candidate (leading to longer trajectories), but outperforms SAC, which found the policy closer to optimal. 
These two results highlight the difference between DRL for GR, compared to traditional DRL tasks. 
Learning a policy with better return does not necessarily lead to a better outcome: it is better to explore and cover more of the state space. 
% Indeed, some exploration to get policy estimations for a larger portion of the state space is desirable. %\reuth{Move the contrastive discussion here?}
% DRACO with the two proposed distance metrics, Wasserstein and Z-score, %, with the Wasserstein distance metric being slightly more informative for the DRACO-SAC variant. 
%
Figures~\ref{fig:panda-f-score-episodes} and~\ref{fig:panda-f-scoreobservability} compare the \DIFdelbegin \DIFdel{three }\DIFdelend approaches under increasing episodes and observability percentage, respectively.
These figures emphasize the superiority of DRACO over GRAQL across the board in continuous environments. \DIFdelbegin \DIFdel{Figure}\DIFdelend \DIFaddbegin \DIFadd{GRAQL performance improves when episodes increase but generalizing a large problem for GRAQL takes a substantially more amount of computations than it takes for DRACO. However, in the partial observation scenario (Figure \ref{fig:panda-f-scoreobservability}), as the observability percentage increases DRACO's performance increases as well while GRAQL's remains about the same emphasizing its inability to learn the problem (even for the 100\% observability problem).
Figure}\DIFaddend ~\ref{fig:noisy_results} illustrates performance under noisy (but complete) observations.\footnote{Supplementary material includes a breakdown of the results.} DRACO outperforms GRAQL with low variance, showing its substantial resilience to noise. \DIFaddbegin \DIFadd{DRACO was barely impacted by the 10\% and 20\% noise ratio preserving its performance from the full-observable non noisy observation.
}\DIFaddend Indeed, the gap between DRACO and GRAQL \textit{increases} as the noise ratio decreases. 
Such a difference in performance is likely due to \DIFdelbegin \DIFdel{the %DIF < \ben{Should we maybe add also because of the distance function?}
richer representation %DIF < of the action options and state 
}\DIFdelend \DIFaddbegin \DIFadd{its leverage of DL to the learning stage and the richer representation state }\DIFaddend available to DRACO.
% In our test environment, overall, DRACO and GRAQL achieve similar results in the discrete environment  high observability. However, in both low observability discrete environments and off-course continuous environments DRACO achieves higher performance with lower variance.
\DIFaddbegin 

\DIFadd{Secondly, Figure \ref{fig:panda-comp} also compares the different evaluation metrics proposed in this paper in section \ref{sec:infer}. Figure \ref{fig:panda-f-score-episodes} shows a slight dominance of DRACO using Wasserstein distance over DRACO using Z-score when trained for <125K, but for 150K+ episodes it turned over.
The number of trained episodes impacts the optimality of the agent making the Z-score metric better for scenarios where the trained agent policy is more optimal.
This happens because the Z-score metric takes into consideration the standard deviation of the policy distribution which takes more episodes to stabilize.
Figures \ref{fig:panda-f-scoreobservability}, \ref{fig:noisy_results} shows a dominance of Wasserstein over Z-score, for observability
levels of < 50\% and with noisy observations.
Wasserstein is better under high uncertainty stemming from the observations, as the Z-score metric is more sensitive to high variability that skews it from the right goal.
}

\DIFaddend To conclude, \DIFdelbegin \DIFdel{DRACO }\DIFdelend \DIFaddbegin \DIFadd{we evaluate the two main contributions of the paper: the DRACO framework and the proposed distance metrics.
First, DRACO is a more scalable solution than the state-of-the-art GR (GRAQL) in both storage consumption and computation time. Beyond that, in terms of the framework performance, DRACO }\DIFaddend achieves better or equal results to GRAQL across the board with much lower variance \DIFdelbegin \DIFdel{. 
}\DIFdelend \DIFaddbegin \DIFadd{in the discrete and continuous environmental setups.
In terms of the different distance metrics, both the Wasserstein and the Z-score distance metrics performed overwhelmingly, however, the former metric was slightly better in less observable spaces and under noise observations.
}


\DIFaddend % In our test environment, DRACO always recognizes the correct goal (exclusively so), and with higher probability.%, for all problems.


%To conclude, these preliminary results exemplify two out of the three different scenarios discussed in this proposal in section \ref{sec:hypotheses}. These results provide initial support to the first and second hypotheses.
%The other hypothesis is yet to be researched in the preliminary results but will further be researched in this work. 
%DIF < \DIFdelbegin %DIFDELCMD < \leo[inline]{%%%
\DIFdel{Removed text referring to Ben's proposal, will later include a conclusion to this section}%DIFDELCMD < } %%%
\DIFdelend %DIF > \leo[inline]{Removed text referring to Ben's proposal, will later include a conclusion to this section}


==> sections/minigrid-table.tex <==
\begin{table*}[tb]
\footnotesize
\scriptsize
\setlength{\tabcolsep}{3pt}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}  
\hline  
& &
 \multicolumn{4}{|c|}{DRACO using KL-Divergence} 
 &
 \multicolumn{4}{|c|}{GRAQL using KL-Divergence}  \\
\hline  
OBS & Problem & Accuracy & Precision & Recall & F-Score & Accuracy & Precision & Recall & F-Score \\ 
\hline  
0.1 & Lava &
\multicolumn{1}{c|}{$\textbf{0.73} \boldsymbol{\pm} \textbf{0.32}$} &
\multicolumn{1}{c|}{$\textbf{0.6} \boldsymbol{\pm} \textbf{0.52}$} &
\multicolumn{1}{c|}{0.6 \textpm\ 0.52} &
\multicolumn{1}{c|}{$\textbf{0.6} \boldsymbol{\pm} \textbf{0.52}$} &
\multicolumn{1}{c|}{0.53 \textpm\ 0.32} &
\multicolumn{1}{c|}{0.41 \textpm\ 0.36} &
\multicolumn{1}{c|}{$\textbf{0.9} \boldsymbol{\pm} \textbf{0.32}$} &
\multicolumn{1}{c|}{0.56 \textpm\ 0.32}
\\  
 & 2-Goals &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{0.7 \textpm\ 0.35} &
\multicolumn{1}{c|}{0.64 \textpm\ 0.35} &
\multicolumn{1}{c|}{0.9 \textpm\ 0.31} &
\multicolumn{1}{c|}{0.75 \textpm\ 0.32}
 \\  
 & 3-Goals &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
\multicolumn{1}{c|}{0.66 \textpm\ 0.35} &
\multicolumn{1}{c|}{0.56 \textpm\ 0.4} &
\multicolumn{1}{c|}{0.9 \textpm\ 0.32} &
\multicolumn{1}{c|}{0.64 \textpm\ 0.35}
 \\  
 \hline  
0.3 & Lava & 
\multicolumn{1}{c|}{$\textbf{0.93}\boldsymbol{\pm} \textbf{0.21}$} &
\multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
\multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
\multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
\multicolumn{1}{c|}{0.87 \textpm\ 0.28} &
\multicolumn{1}{c|}{0.8 \textpm\ 0.42} &
\multicolumn{1}{c|}{0.8 \textpm\ 0.42} &
\multicolumn{1}{c|}{0.8 \textpm\ 0.42}
\\  
 & 2-Goals & 
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$}
 \\  
 & 3-Goals &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
 \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$}
 \\ 
%  \hline  
% 0.5 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\
% & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
% & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
% \hline  
% 0.7 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
%  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
%  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
% \hline  
% 1.0 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
%  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
%  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
% \hline 
% Noisy & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
%  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
%  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
\hline 
\end{tabular}
    \caption{
        Impact of partial observability, KL-Divergence is used to measure the distance between the optimal paths and the given observation in both approaches. The results are the average (± standard deviation) of 10 different executions.
    }
    \label{tab:minigrid}
\end{table*}


==> sections/minigrid-tables2.tex <==
\begin{table*}[tb]
\begin{subtable}[b]{0.3\textwidth}
    \centering
    \small
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|} 
    \cline{2-9}
    \multicolumn{1}{c|}{} & \multicolumn{4}{c|}{GRAQL}                     & \multicolumn{4}{c|}{DRACO}                      \\ 
    \cline{2-9}
    \multicolumn{1}{l|}{} & $\alpha$ & $\epsilon$ & $\gamma$ & Epis. & $\alpha$ & $\epsilon$ & $\gamma$ & Epis.  \\ 
    \hline
    Minigrid              & $1e^{-3}$      & $1.5e^{-7}$     & $0.93$       & $50k$   & $1e^{-3}$      & $1e^{-6}$     & $0.93$       & $25k$    \\ 
    \hline
    Panda-Gym             & $1e^{-4}$     & $0.3$          & $0.99$       & $100k$  & $1e^{-4}$     & $0.3$          & $0.99$       & $100k$   \\
    \hline
    \end{tabular}
    \normalsize
    \caption{Hyperparameters for Experimentation}
    \label{tab:hyperparameters}
\end{subtable}
\begin{subtable}[b]{0.7\textwidth}
    \footnotesize
    \scriptsize
    \setlength{\tabcolsep}{3pt}
        \centering
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}  
    \hline  
    & &
     \multicolumn{4}{|c|}{DRACO using KL-Divergence} 
     &
     \multicolumn{4}{|c|}{GRAQL using KL-Divergence}  \\
    \hline  
    OBS & Problem & Accuracy & Precision & Recall & F-Score & Accuracy & Precision & Recall & F-Score \\ 
    \hline  
    0.1 & Lava &
    \multicolumn{1}{c|}{$\textbf{0.73} \boldsymbol{\pm} \textbf{0.32}$} &
    \multicolumn{1}{c|}{$\textbf{0.6} \boldsymbol{\pm} \textbf{0.52}$} &
    \multicolumn{1}{c|}{0.6 \textpm\ 0.52} &
    \multicolumn{1}{c|}{$\textbf{0.6} \boldsymbol{\pm} \textbf{0.52}$} &
    \multicolumn{1}{c|}{0.53 \textpm\ 0.32} &
    \multicolumn{1}{c|}{0.41 \textpm\ 0.36} &
    \multicolumn{1}{c|}{$\textbf{0.9} \boldsymbol{\pm} \textbf{0.32}$} &
    \multicolumn{1}{c|}{0.56 \textpm\ 0.32}
    \\  
     & 2-Goals &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{0.7 \textpm\ 0.35} &
    \multicolumn{1}{c|}{0.64 \textpm\ 0.35} &
    \multicolumn{1}{c|}{0.9 \textpm\ 0.31} &
    \multicolumn{1}{c|}{0.75 \textpm\ 0.32}
     \\  
     & 3-Goals &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
    \multicolumn{1}{c|}{0.66 \textpm\ 0.35} &
    \multicolumn{1}{c|}{0.56 \textpm\ 0.4} &
    \multicolumn{1}{c|}{0.9 \textpm\ 0.32} &
    \multicolumn{1}{c|}{0.64 \textpm\ 0.35}
     \\  
     \hline  
    0.3 & Lava & 
    \multicolumn{1}{c|}{$\textbf{0.93}\boldsymbol{\pm} \textbf{0.21}$} &
    \multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
    \multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
    \multicolumn{1}{c|}{$\textbf{0.9}\boldsymbol{\pm} \textbf{0.31}$} &
    \multicolumn{1}{c|}{0.87 \textpm\ 0.28} &
    \multicolumn{1}{c|}{0.8 \textpm\ 0.42} &
    \multicolumn{1}{c|}{0.8 \textpm\ 0.42} &
    \multicolumn{1}{c|}{0.8 \textpm\ 0.42}
    \\  
     & 2-Goals & 
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$}
     \\  
     & 3-Goals &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$} &
     \multicolumn{1}{c|}{$\textbf{1.0}\boldsymbol{\pm} \textbf{0.0}$}
     \\ 
    %  \hline  
    % 0.5 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\
    % & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    % & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    % \hline  
    % 0.7 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
    %  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    %  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    % \hline  
    % 1.0 & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
    %  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    %  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    % \hline 
    % Noisy & Lava & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
    %  & 2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    %  & 3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
    \hline 
    \end{tabular}
        \caption{
            Impact of partial observability, KL-Divergence is used to measure the distance between the optimal paths and the given observation in both approaches. The results are the average (± standard deviation) of 10 different executions.
        }
        \label{tab:minigrid}
\end{subtable}
\end{table*}

==> sections/partial_obs.tex <==
% !TEX root = ../main.tex
\begin{center}
\begin{table*}[h]
\footnotesize
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}  
\hline  
& &
 \multicolumn{4}{|c|}{GRDRL} 
 &
 \multicolumn{4}{|c|}{GRAQL}  \\
\hline  
OBS & Problem & Accuracy & Precision & Recall & F-Score & Accuracy & Precision & Recall & F-Score \\ 
\hline  
0.1 & Lava-Grid-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 0.93 & 0.9 & 0.9 & 0.9 \\  
 & Empty-2-Goals & 1.0  & 1.0 & 1.0 & 1.0 & 0.8 & 0.8 & 0.8 & 0.8\\  
 & Empty-3-Goals & 1.0  & 1.0 & 1.0 & 1.0 & 0.93 & 0.9 & 0.9 & 0.9\\  
 \hline  
0.3 & Lava-Grid-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
 & Empty-2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 0.8 & 0.9 & 0.9 & 0.9\\  
 & Empty-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
 \hline  
0.5 & Lava-Grid-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\
& Empty-2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
& Empty-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
\hline  
0.7 & Lava-Grid-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
 & Empty-2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
 & Empty-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
\hline  
1.0 & Lava-Grid-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0\\  
 & Empty-2-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
 & Empty-3-Goals & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0\\ 
\hline  
\end{tabular}
    \caption{
        Impact of partial observability and noise on both frameworks, KL is used to measure the distance between the optimal paths and the given observation. The results are the average of 10 different executions.
    }
    \label{tab:my_label}
\end{table*}
\end{center}
